Testing by Dualization

Software engineering requires rigorous testing to guarantee the product's quality. Semantic testing of functional correctness is challenged by nondeterminism in behavior, which makes testers difficult to write and reason about. This thesis presents a language-based technique for testing interactive systems. I propose a theory for specifying and validating nondeterministic behaviors, with guaranteed soundness and correctness. I then apply the theory to testing practices, and show how to derive specifications into interactive tester programs. I also introduce a language design for producing test inputs that can effectively detect and reproduce invalid behaviors. I evaluate the methodology by specifying and testing real-world systems such as web servers and file synchronizers, demonstrating the derived testers' ability to find disagreements between the specification and the implementation.

==> Makefile <==
all: thesis.pdf

%.pdf:
	latexmk -pdf -file-line-error -halt-on-error -interaction=nonstopmode \
		-outdir=docs $*

clean:
	latexmk -C -outdir=docs
	$(RM) *~


==> math-proof.tex <==
\section{Forward preservation lemma for rejection soundness}
\label{sec:rs2-proof}
\autoref{eq:rs2}

\begin{align*}
  &\forall(p:\Prog)(q,c,a:\Int)(s_0,s':\sigma)(v:\beta),\\
  &\sstep_p(q,c,s_0)=(a,s')\wedge\Reflects{v}{s_0}\\
  &\implies\exists v':\beta,\vstep_p(q,a,v)=\Some{v'}\wedge\Reflects{v'}{s'}
\end{align*}

The invariant $\Reflects{v}{s_0}$ tells us that $v$ contains a validation state
that reflects the server state $s_0$:
\[\exists((vs_0,cs_0)\in v)(asgn_0:\Var\to\Int),\satisfy{asgn_0} cs_0\wedge {vs_0}^{asgn_0}\equiv s_0\]

The corresponding validator step is constructed by analyzing the server step,
and proving small-step bisimulation for each derivation rule
in \autoref{sec:dualization}.

\paragraph{Write}
The server writes some expression $(e:\Sexp)$ to an address $!dst$.
According to \autoref{rule:write}, the validator creates a fresh variable $x_e$
for address $!dst$, and constraints that $(\#x_e\equiv e^{vs})$.\footnote{If
unspecified, $(vs,cs)$ represents the pre-small-step validator state, and $s$
represents the pre-small-step server state.}

We need to show that:
\begin{align*}
&\forall vs,cs,s,asgn,\\
&\satisfy{asgn}{cs}\wedge vs^{asgn}\equiv s\\
&\implies\forall d,e,\begin{array}[t]{lll}
\letin{s'&}{\update{s}{d}{e^s}&}\\
\letin{(vs',cs')&}{\Write(d,e,(vs,cs))&}\\
\multicolumn{3}{l}{\exists asgn',\quad\satisfy{asgn'}{cs'}\wedge vs'^{~asgn'}\equiv s'}
\end{array}
\end{align*}
\begin{proof}
Based on the definition of $\Write$, we need to show that:
\begin{align*}&\letin{x_e}{\Fresh(vs,cs)}\\
&\letin{vs'}{\update{vs}{d}{x_e}}\\
&\letin{cs'}{cs\cup\{x_e\equiv e^{vs}\}}\\
&\exists asgn',\quad\satisfy{asgn'}{cs'}\wedge vs'^{~asgn'}\equiv s'
\end{align*}
Let:\[asgn'=\update{asgn}{x_e}{e^{s}}\]

In order to prove $(\satisfy{asgn'}{cs'})$, we introduce some generic lemmas to
show that $(\satisfy{asgn'}{cs})$ and $({x_e}^{asgn'}\equiv{(e^{vs})^{asgn'}})$:
\begin{lemma}[Fresh variable preserves satisfaction]
\label{lem:fresh-sat}
\begin{align*}
&\forall (cs:\Set\constraint)(asgn:\Var\to\Int),\\
&\satisfy{asgn}{cs}\\
&\implies
\begin{array}[t]{lll}
\multicolumn{3}{l}{\forall (z:\Int),vs,}\\
\letin{x&}{\Fresh(vs,cs)&}\\
\letin{asgn'&}{\update{asgn}{x}{z}&}\\
\multicolumn{3}{l}{\satisfy{asgn'}{cs}}
\end{array}
\end{align*}
\begin{proof}
Since $x$ is fresh in $cs$, we have:
\[\forall (e_1\ccmp e_2)\in cs,\quad{e_1}^{asgn'}={e_1}^{asgn}\wedge{e_2}^{asgn'}={e_2}^{asgn}\]

Thus:
\begin{align*}
&\forall (e_1\ccmp e_2)\in cs,\quad{e_1}^{asgn'}\ccmp {e_2}^{asgn'}\\
&\textit{i.e. }\satisfy{asgn'} cs
\end{align*}
\end{proof}
\end{lemma}

\begin{lemma}[Fresh variable preserves evaluation]
\label{lem:fresh-eval}
\begin{align*}
&\forall (vs:\Nat\to\Var)(asgn:\Var\to\Int)(z:\Int),cs,\\
&\begin{array}[t]{lll}
\letin{x&}{\Fresh(vs,cs)&}\\
\letin{asgn'&}{\update{asgn}{x}{z}&}\\
\multicolumn{3}{l}{\forall (e:\Sexp),(e^{vs})^{asgn'}=(e^{vs})^{asgn}}
\end{array}
\end{align*}
\begin{proof}
Assume to the contrary that: \[(e^{vs})^{asgn'}\neq(e^{vs})^{asgn}\]

Since $asgn'$ is the same as $asgn$ except for variable $\#x$, we know that
$(e^{vs}:\Vexp)$ must involve $\#x$.  Therefore, $e$ must involve some address
$!k$ such that $(vs!k=x)$.  This contradicts the fact that $x$ is fresh in $vs$.
\end{proof}
\end{lemma}

\begin{lemma}[Symbolization preserves evaluation]
\label{lem:sym-eval}
\begin{align*}
&\forall(vs:\Nat\to\Var)(asgn:\Var\to\Int)(s:\Nat\to\Int),\\
&vs^{asgn}\equiv s\implies\forall (e:\Sexp),\quad(e^{vs})^{asgn}\equiv e^s
\end{align*}
\begin{proof}
Based on the definition of symbolization and evaluation:
\begin{itemize}
\item $e^{vs}$ substitutes all occurences of $!k$ in $e$ with $\#(vs!k)$;
\item $(e^{vs})^{asgn}$ substitutes all occurences of $\#(vs!k)$ to $asgn!(vs!k)$;
\item $e^s$ substitutes all occurences of $!k$ in $e$ with $(s!k)$.
\end{itemize}

From the hypothesis that $(vs^{asgn}\equiv s)$, we have:
\[\forall (k:\Nat),\quad asgn!(vs!k)\equiv (s!k)\]

Therefore, we know that all occurences of $!k$ were mapped to the same value
between the two evaluation paths.
\end{proof}
\end{lemma}

Based on \autoref{lem:fresh-eval}, we have:
\[{(e^{vs})}^{asgn'}={(e^{vs})}^{asgn}\]



Also, since $x_e$ is free in $vs$, and $asgn'$ is the same as $asgn$ except for
$x_e$, we have:
\[\forall k,asgn'!(vs'!k)=\begin{cases}
asgn'!x_e=e^s=(s'!k)&k\Is d\\
asgn!(vs!k)=(s!k)=(s'!k)&\text{otherwise}
\end{cases}\]
Therefore:\[vs'^{~asgn'}\equiv s'\]
\end{proof}

\paragraph{Havoc}
When the server writes some internal choice $c$ to address $d$,
according to \autoref{rule:choice}, the validator creates a fresh variable for
address $!d$.

We need to show that:
\begin{align*}&\forall vs,cs,s,asgn,\\
&\satisfy{asgn}{cs}\wedge vs^{asgn'}\equiv s\\
&\implies\forall d,c,\begin{array}[t]{lll}
\letin{s'&}{\update{s}{d}{c}&}\\
\letin{x_c&}{\Fresh(vs,cs)&}\\
\multicolumn{3}{l}{\exists asgn',\quad\satisfy{asgn'} cs\wedge vs^{asgn'}\equiv s'}
\end{array}
\end{align*}
\begin{proof}
Let:\[asgn'=\update{asgn}{x_c}{c}\]
Since $x_c$ is free in $cs$, we have
\end{proof}

%% \[\havoc(d,(vs,cs))=\letin{x_c}{\Fresh(vs,cs)}{(\update{vs}{d}{x_c},cs)}\]

%% \begin{proof}
%% We can construct the following assignment:
%% \[asgn_1=\update{asgn_0}{x_c}{c}\]


%% Since $x_c$ is also fresh in $vs_0$, we have:
%% \[\forall addr, asgn_1!(vs_1!addr)=\begin{cases}
%% asgn_1!x_c=c\equiv s_1!addr&addr\Is1\\
%% asgn_0!(vs_0!addr)=s_0!addr\equiv s_1!addr&\text{otherwise}
%% \end{cases}\]

%% Thus: \[{vs_1}^{asgn_1}\equiv s_1\]
%% \end{proof}

\section{Backward preservation lemma for rejection completeness}
\label{sec:rc2-proof}

\autoref{eq:rc2}


==> motivation.tex <==
The Deep Specification project~\cite{deepspec} aims at building a web server and
guarantee its functional correctness with respect to formal specification of the
network protocol.

It is possible, but tricky, to write an ad hoc tester for \http by manually
``dualizing'' the behaviors described by the informal specification documents
(RFCs).  The protocol document describes {\em how} a valid server should handle
requests, while the tester needs to determine {\em what} responses received from
the server are valid.  For example, ``If the server has revealed some resource's
ETag as \inlinec{"foo"}, then it must not reject requests targetting this
resource conditioned over \inlinec{If-Match: "foo"}, until the resource has been
modified''; and ``Had the server previously rejected an \inlinec{If-Match}
request, it must reject the same request until its target has been modified.''
\autoref{fig:etag-tester} shows a hand-written tester for checking this bit of
ETag functionality; we hope the reader will agree that this testing logic is not
straightforward to derive from the informal ``server's eye'' specifications.

Networked systems are naturally concurrent, as a server can be connected with
multiple clients.  The network might delay packets indefinitely, so messages
sent via different channels may be reordered during transmission.  When the
tester observes messages sent and received on the client side, it should allow
all observations that can be explained by the combination of a valid server + a
reasonable network environment between the server and clients.

